Fireball characteristics derivable from acoustic data

Near field acoustical signals from fireballs (ranges<200 km), when detected by dense ground networks, may be used to estimate the orientation of the trajectory of a fireball (Pujol et al., 2005) as well as fragmentation locations (Kalenda et al., 2014; Edwards and Hildebrand, 2004). Distinguishing ballistic arrivals (from the cylindrical shock of the fireball)from fragmentation generated signals (quasi-spherical sources) remains a challenge, but are obtainable through analysis of the acoustic path and the timing observed at ground instruments. Here we describe an integrated computer code, termed the Bolide Acoustic Modelling program or BAM, to estimate fireball trajectories and energetics. We develop a new methodology for measuring energy release from bolide fragmentation episodes solely from acoustic measurements and incorporate this into BAM. We also explore the sensitivity of seismo-acoustic fireball solutions and energy estimates to uncertainty in the underlying atmospheric model. Applying BAM to the Stubenberg meteorite producing fireball, we find the total fireball energy from ballistic arrivals to be approximately $5 \times 10^{10}$J which compares favorably to the optical estimate of $4.36 \times 10^{10}$J. The combined fragmentation energy of the Stubenberg event from acoustic data was found to be $1.47^{+0.28}_{-0.12} \times 10^{10}$J, roughly one third of the ballistic or optical total energy. We also show that measuring fireball velocities from acoustic data alone is very challenging but may be possible for slow, deeply penetrating fireballs with shallow entry angles occurring over dense seismic/infrasound networks.

==> removed-text-oct-16-2019 <==

\subsection{Theoretical Fireballs}
Artificial fireballs will be simulated by the program with varying zenith angles and velocities to determine the differences in arrival times for certain geometries. How well the timing of the fireball can be resolved if it were to travel at varying velocities will be studied. If it is found that fireballs of different velocities create arrival times at a station which differ on the order of seconds, then it may be possible for that geometry to solve for the velocity directly, using acoustic data alone. 

\subsection{Theoretical Fireballs}
The Stubenberg meteor will be tweaked to create artificial meteors in the same area. Meteors with the same initial conditions, but varying velocities and zenith angles will be simulated from this release. Rays will be traced for the ballistic solution from each trajectory, and the arrival times of each unique trajectory will be compared, specifically, how the arrival times depend on velocity. 
